Multi-agent Time-based Decision-making for the Search and Action Problem

Many robotic applications, such as search-and-rescue, require multiple agents to search for and perform actions on targets. However, such missions present several challenges, including cooperative exploration, task selection and allocation, time limitations, and computational complexity. To address this, we propose a decentralized multi-agent decision-making framework for the search and action problem with time constraints. The main idea is to treat time as an allocated budget in a setting where each agent action incurs a time cost and yields a certain reward. Our approach leverages probabilistic reasoning to make near-optimal decisions leading to maximized reward. We evaluate our method in the search, pick, and place scenario of the Mohamed Bin Zayed International Robotics Challenge (MBZIRC), by using a probability density map and reward prediction function to assess actions. Extensive simulations show that our algorithm outperforms benchmark strategies, and we demonstrate system integration in a Gazebo-based environment, validating the framework's readiness for field application.

==> Makefile <==
## Makefile to compile .tex files.
#
# Author: Gregory Hitz
#

## targets and dependencies
# by default all .tex will be converted into .pdf:
#targets=$(subst .tex,.pdf,$(wildcard *.tex))
targets=2018-icra-miki.pdf

# definition of dependency directories
images_dir = images
ref_dir = references


# compilation feature switches. Should be 0 (off) or 1 (on). If the variables
# are set as environmnet variables they are read from there. otherwise the
# default values are assigned (after the minus sign)
# use_gs:				use ghostscript to postprocess the compiled pdf
#						(default = 1)
# fail_on_missing_refs: fail if pdflatex reports missing references
#						(default = 0)
# These settings can also be applied as arguments to the make call:
#		(e.g.: $ make use_gs=1)
# NOTE:	for this to work the env variables need to be exported
#		(e.g.: export USE_GS=1;)
use_gs = $(shell echo $${USE_GS:-1})
fail_on_missing_refs =  $(shell echo $${FAIL_ON_MISSING_REFS:-0})
refold = $(shell echo $${refold:-HEAD~1})
refnew = $(shell echo $${refnew:-HEAD})

deps= \
	  $(wildcard *.inc) \
	  $(wildcard $(images_dir)/*.pdf) $(wildcard $(images_dir)/**/*.pdf) \
	  $(wildcard images/*.jpg) $(wildcard $(images_dir)/**/*.jpg) \
	  $(wildcard $(images_dir)/*.png) $(wildcard $(images_dir)/**/*.png) \
	  $(wildcard *.sty) \
	  Makefile
bib= \
	 $(wildcard $(ref_dir)/*.bib) $(wildcard $(ref_dir)/**/.bib)


all: $(targets) 

%.pdf: %.tex $(bib) $(deps) | build
	date > build/buildlog_$@.txt;
	printf "compling $@\n" >> build/buildlog_$@.txt
	# first we run pdflatex
	cd build && TEXINPUTS=..:${TEXINPUTS} pdflatex -draftmode ../$<
	# now we need to know if we need to run bibtex or bib. For this we check if
	# the aux file contains cite commands. If so we check if there is a bcf
	# file, in which case we run biber. otherwise we run bibtex.
	cd build; \
	if grep -qE "citation\{|cite\{" $(subst .pdf,.aux,$@); then \
	printf "$@: compiling biblio with " | tee -a buildlog_$@.txt; \
	if [ -f $(subst .pdf,.bcf,$@) ]; then \
	printf "biber\n" | tee -a buildlog_$@.txt; \
	biber --input-directory=.. $(subst .pdf,,$@); \
	else \
	printf "bibtex\n" | tee -a buildlog_$@.txt; \
	BIBINPUTS=..:${BIBINPUTS} BSTINPUTS=..:${BSTINPUTS} \
	bibtex $(subst .pdf,,$@); \
	fi; \
	TEXINPUTS=..:${TEXINPUTS} pdflatex -draftmode ../$<; \
	else \
	printf "$@: no biblio\n" | tee -a buildlog_$@.txt; \
	fi;
	cd build && TEXINPUTS=..:${TEXINPUTS} pdflatex ../$< 
	# the pdf should be complete at this point. ideally we use gs now to get
	# the images to reasonable sizes. if not we just move it to the main
	# directory
	if [ $(use_gs) = 1 ]; then \
	printf "Running ghostscript\n" | tee -a build/buildlog_$@.txt; \
	gs -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -dPDFSETTINGS=/prepress \
	-sOutputFile=$@ build/$@ || mv build/$@ .; \
	du -sh $@ build/$@; \
	else \
	printf "No ghostscript\n" | tee -a build/buildlog_$@.txt; \
	mv build/$@ . ; \
	fi;
	@if [ $(fail_on_missing_refs) = 1 ]; then \
	printf "I'll fail on missing reference ...\n" | tee -a build/buildlog_$@.txt; \
	if (grep "There were undefined references\|citations" build/$(subst .pdf,.log,$@) \
	 || grep "biblatex Warning: The following entry could not be found" \
	 build/$(subst .pdf,.log,$@) ); then \
	printf "BUILD FAILED because of undefined references or citations in $<\n" | \
	tee -a build/buildlog_$@.txt; \
	false; \
	else \
	printf "BUILD SUCEEDED There were no undefined references or citations\n" | \
	tee -a build/buildlog_$@.txt; \
	fi; \
	else printf "Not checking for undefined references or citations\n" | \
	tee -a build/buildlog_$@.txt; \
	fi;

test:
	echo "cloning and testing in: $$TMPDIR/temp_test_dir"
	rm -rf $$TMPDIR/temp_test_dir
	curdir=$$(pwd) && \
	cd $$TMPDIR && \
	git clone "$$curdir" temp_test_dir && \
	cd temp_test_dir && \
	make use_gs=$(use_gs) fail_on_missing_refs=$(fail_on_missing_refs)
	@echo "successfully tested in: $$TMPDIR/temp_test_dir"

diff.tex: build
	git show $(refold):$(subst .pdf,.tex,$(targets)) > build/old.tex \
		&& git show $(refnew):$(subst .pdf,.tex,$(targets)) > build/new.tex \
		&& latexdiff --disable-citation-markup --exclude-textcmd="section,subsection" \
		--math-markup=0 build/old.tex \
		build/new.tex > diff.tex
	#rm build/old.tex
	#rm build/new.tex


diff: diff.pdf

build:
	mkdir -p build

debug:
	@echo "--- Evironment variables ------------------"
	@echo "USE_GS: $$USE_GS"
	@echo "FAIL_ON_MISSING_REFS: $$FAIL_ON_MISSING_REFS"
	@echo "--- Switches ------------------------------"
	@echo "use_gs: $(use_gs)"
	@echo "fail_on_missing_refs: $(fail_on_missing_refs)"
	@echo "--- Targets -------------------------------"
	@echo $(targets) | tr " " "\n"
	@echo "--- Bibs ----------------------------------"
	@echo $(bib) | tr " " "\n"
	@echo "--- Deps ----------------------------------"
	@echo $(deps) | tr " " "\n"
	@echo "--- Diff points ----------------------------------"
	@echo "ref old: $(refold)" 
	@echo "ref new: $(refnew)" 

clean: buildclean

buildclean:
	rm -rf build  

distclean: buildclean
	rm -f $(targets)

.PHONY: all clean buildclean distclean debug test diff



==> chapters/abstract.tex <==
\chapter*{Abstract}
\addcontentsline{toc}{chapter}{Abstract}
%\chapter*{Zusammenfassung}
%\addcontentsline{toc}{chapter}{Zusammenfassung}

Hier kommt der Abstact hin \dots

==> chapters/chapter.tex <==
\chapter{Einige wichtige Hinweise zum Arbeiten mit \LaTeX\ }
\label{sec:latexumg}

Nachfolgend wird die Codierung einiger oft verwendeten Elemente
kurz beschrieben. Das Einbinden von Bildern ist in \LaTeX\ nicht
ganz unproblematisch und hängt auch stark vom verwendeten Compiler
ab. Typisches Format für Bilder in \LaTeX\ ist
EPS\footnote{Encapsulated Postscript} oder PDF\footnote{Portable Document Format}.


\section{Gliederungen}
\label{sec:gliederung}

Ein Text kann mit den Befehlen \texttt{\textbackslash
chapter\{.\}}, \texttt{\textbackslash section\{.\}},
\texttt{\textbackslash subsection\{.\}} und \texttt{\textbackslash
subsubsection\{.\}} gegliedert werden.


\section{Referenzen und Verweise}
\label{sec:refverw}

Literaturreferenzen werden mit dem Befehl \texttt{\textbackslash
citep\{.\}} und \texttt{\textbackslash
citet\{.\}} erzeugt. Beispiele: ein Buch \citep{Raibert1986LeggedRobotsThatBalance}, ein Buch und ein Journal Paper \citep{Raibert1986LeggedRobotsThatBalance,Vukobratovic2004ZeroMomentPoint}, ein Konferenz Paper mit Erwähnung des Autors: \citet{Pratt1995SEA}.

Zur Erzeugung von Fussnoten wird der Befehl \texttt{\textbackslash
footnote\{.\}} verwendet. Auch hier ein Beispiel\footnote{Bla
bla.}.

Querverweise im Text werden mit \texttt{\textbackslash label\{.\}}
verankert und mit \texttt{\textbackslash cref\{.\}} erzeugt.
Beispiel einer Referenz auf das zweite Kapitel:
\cref{sec:latexumg}.


\section{Aufzählungen}\label{sec:aufz}

Folgendes Beispiel einer Aufzählung ohne Numerierung,
\begin{itemize}
  \item Punkt 1
  \item Punkt 2
\end{itemize}
wurde erzeugt mit:
\begin{verbatim}
\begin{itemize}
  \item Punkt 1
  \item Punkt 2
\end{itemize}
\end{verbatim}

Folgendes Beispiel einer Aufzählung mit Numerierung,
\begin{enumerate}
  \item Punkt 1
  \item Punkt 2
\end{enumerate}
wurde erzeugt mit:
\begin{verbatim}
\begin{enumerate}
  \item Punkt 1
  \item Punkt 2
\end{enumerate}
\end{verbatim}

Folgendes Beispiel einer Auflistung,
\begin{description}
  \item[P1] Punkt 1
  \item[P2] Punkt 2
\end{description}
wurde erzeugt mit:
\begin{verbatim}
\begin{description}
  \item[P1] Punkt 1
  \item[P2] Punkt 2
\end{description}
\end{verbatim}


\section{Erstellen einer Tabelle}\label{sec:tabellen}

Ein Beispiel einer Tabelle:
\begin{table}[h]
\begin{center}
 \caption{Daten der Fahrzyklen ECE, EUDC, NEFZ.}\vspace{1ex}
 \label{tab:tabnefz}
 \begin{tabular}{ll|ccc}
 \hline
 Kennzahl & Einheit & ECE & EUDC & NEFZ \\ \hline \hline
 Dauer & s & 780 & 400 & 1180 \\
 Distanz & km & 4.052 & 6.955 & 11.007 \\
 Durchschnittsgeschwindigkeit & km/h & 18.7 &  62.6 & 33.6 \\
 Leerlaufanteil & \% & 36 & 10 & 27 \\
 \hline
 \end{tabular}
\end{center}
\end{table}

Die Tabelle wurde erzeugt mit:
\begin{verbatim}
\begin{table}[h]
\begin{center}
 \caption{Daten der Fahrzyklen ECE, EUDC, NEFZ.}\vspace{1ex}
 \label{tab:tabnefz}
 \begin{tabular}{ll|ccc}
 \hline
 Kennzahl & Einheit & ECE & EUDC & NEFZ \\ \hline \hline
 Dauer & s & 780 & 400 & 1180 \\
 Distanz & km & 4.052 & 6.955 & 11.007 \\
 Durchschnittsgeschwindigkeit & km/h & 18.7 &  62.6 & 33.6 \\
 Leerlaufanteil & \% & 36 & 10 & 27 \\
 \hline
 \end{tabular}
\end{center}
\end{table}
\end{verbatim}


\section{Einbinden einer Grafik}\label{sec:epsgraph}

Das Einbinden von Graphiken kann wie folgt bewerkstelligt werden:
\begin{verbatim}
\begin{figure}
   \centering
   \includegraphics[width=0.75\textwidth]{images/k_surf.pdf}
   \caption{Ein Bild.}
   \label{fig:k_surf}
\end{figure}
\end{verbatim}

\begin{figure}
   \centering
   \includegraphics[width=0.75\textwidth]{images/k_surf.pdf}
   \caption{Ein Bild}
   \label{pics:k_surf}
\end{figure}

oder bei zwei Bildern nebeneinander mit:
\begin{verbatim}
\begin{figure}
  \begin{minipage}[t]{0.48\textwidth}
    \includegraphics[width = \textwidth]{images/cycle_we.pdf}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.48\textwidth}
    \includegraphics[width = \textwidth]{images/cycle_ml.pdf}
  \end{minipage}
  \caption{Zwei Bilder nebeneinander.}
  \label{pics:cycle}
\end{figure}
\end{verbatim}

\begin{figure}
  \begin{minipage}[t]{0.48\textwidth}
    \includegraphics[width = \textwidth]{images/cycle_we.pdf}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.48\textwidth}
    \includegraphics[width = \textwidth]{images/cycle_ml.pdf}
  \end{minipage}
  \caption{Zwei Bilder nebeneinander}
  \label{pics:cycle}
\end{figure}


\section{Mathematische Formeln}\label{sec:math}

Einfache mathematische Formeln werden mit der equation-Umgebung
erzeugt:
\begin{equation}
 p_{me0f}(T_e,\omega_e) \ = \ k_1(T_e) \cdot (k_2+k_3 S^2
 \omega_e^2) \cdot \Pi_{\mathrm{max}} \cdot \sqrt{\frac{k_4}{B}} \, .
 	\label{eq:my_equation}
\end{equation}

Der Code dazu lautet:
\begin{verbatim}
\begin{equation}
 p_{me0f}(T_e,\omega_e) \ = \ k_1(T_e) \cdot (k_2+k_3 S^2
 \omega_e^2) \cdot \Pi_{max} \cdot \sqrt{\frac{k_4}{B}} \, .
\end{equation}
\end{verbatim}

Mathematische Ausdrücke im Text werden mit \$formel\$ erzeugt (z.B.:
$a^2+b^2=c^2$).

Vektoren und Matrizen werden mit den Befehlen \texttt{\textbackslash vec\{.\}} und \texttt{\textbackslash mat\{.\}} erzeugt (z.B. $\vec{v}$, $\mat{M}$).


\section{Weitere nützliche Befehle}\label{sec:div}

Hervorhebungen im Text sehen so aus: \emph{hervorgehoben}. Erzeugt
werden sie mit dem \texttt{\textbackslash epmh\{.\}} Befehl.

Einheiten werden mit den Befehlen \texttt{\textbackslash unit[1]\{m\}} (z.B.~\unit[1]{m}) und \texttt{\textbackslash unitfrac[1]\{m\}\{s\}} (z.B.~\unitfrac[1]{m}{s}) gesetzt.

